Traceability Support for Multi-Lingual Software Projects

Software traceability establishes associations between diverse software artifacts such as requirements, design, code, and test cases. Due to the non-trivial costs of manually creating and maintaining links, many researchers have proposed automated approaches based on information retrieval techniques. However, many globally distributed software projects produce software artifacts written in two or more languages. The use of intermingled languages reduces the efficacy of automated tracing solutions. In this paper, we first analyze and discuss patterns of intermingled language use across multiple projects, and then evaluate several different tracing algorithms including the Vector Space Model (VSM), Latent Semantic Indexing (LSI), Latent Dirichlet Allocation (LDA), and various models that combine mono- and cross-lingual word embeddings with the Generative Vector Space Model (GVSM). Based on an analysis of 14 Chinese-English projects, our results show that best performance is achieved using mono-lingual word embeddings integrated into GVSM with machine translation as a preprocessing step.

==> tables/exp2_table_back.tex <==

\begin{table}[ht!]

    \centering
     \caption{Result of applying models on intermingled-bilingual dataset and translated monolingual dataset}
        \begin{tabular}{cc cccccc}
        \toprule
        & & \multicolumn{3}{c}{ Intermingled } & \multicolumn{3}{c}{ Translated } \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
        & & CLWE-G & LDA & VSM & WE-G & LDA & VSM \\
         \midrule
        \multirow{2}{*}{ Ar } & F2 & .356 & .240 & .318 & \textbf{.365} & .236 & .317 \\
        & AP & .252 & .112 & .262 & \textbf{.263} & .083 & .259 \\ \midrule
        \multirow{2}{*}{ Ca } & F2 & .250 & .173 & .248 & \textbf{.273} & .156 & .253 \\
        & AP & \textbf{.163} & .046 & .120 & .124 & .053 & .128 \\ \midrule
        \multirow{2}{*}{ Dr } & F2 & .271 & .090 & .275 & \textbf{.313} & .108 & .311 \\
        & AP & .138 & .017 & .196 & .183 & .022 & \textbf{.230} \\ \midrule
        \multirow{2}{*}{ Na } & F2 & .247 & .220 & .251 & \textbf{.294} & .185 & .210 \\
        & AP & \textbf{.132} & .070 & .119 & \textbf{.132} & .054 & .103 \\ \midrule
        \multirow{2}{*}{ Ra } & F2 & .271 & .166 & .253 & \textbf{.311} & .156 & .291 \\
        & AP & .213 & .036 & .160 & \textbf{.230} & .044 & .186 \\ \midrule
        \multirow{2}{*}{ Sa } & F2 & .357 & .294 & .413 & \textbf{.464} & .294 & .413 \\
        & AP & .243 & .074 & \textbf{.382} & .379 & .149 & .360 \\ \midrule
        \multirow{2}{*}{ ER } & F2 & .390 & .236 & .367 & \textbf{.422} & .189 & .362 \\
        & AP & \textbf{.366} & .071 & .232 & .363 & .053 & .227 \\ \midrule
        \multirow{2}{*}{ Em } & F2 & .316 & .263 & .309 & .410 & .263 & \textbf{.430} \\
        & AP & .180 & .066 & \textbf{.172} & .167 & .109 & .160 \\ \midrule
        \multirow{2}{*}{ Bk } & F2 & .116 & .037 & .103 & \textbf{.132} & .059 & .131 \\
        & AP & .033 & .005 & .029 & .036 & .009 & \textbf{.044} \\ \midrule
        \multirow{2}{*}{ Nc } & F2 & .388 & .171 & .346 & \textbf{.429} & .213 & .352 \\
        & AP & .353 & .071 & .329 & \textbf{.388} & .069 & .361 \\ \midrule
        \multirow{2}{*}{ QMA } & F2 & .332 & .164 & .324 & \textbf{.358} & .229 & .348 \\
        & AP & .251 & .051 & .207 & \textbf{.259} & .056 & \textbf{.259} \\ \midrule
        \multirow{2}{*}{ QMI } & F2 & .747 & .278 & .670 & \textbf{.761} & .600 & .707 \\
        & AP & .718 & .215 & .637 & \textbf{.773} & .555 & .666 \\ \midrule
        \multirow{2}{*}{ We } & F2 & \textbf{.289} & .111 & .244 & .259 & .168 & .264 \\
        & AP & \textbf{.209} & .030 & .140 & .160 & .044 & .135 \\ \midrule
        \multirow{2}{*}{ xL } & F2 & \textbf{.560} & .208 & .427 & .489 & .208 & .464 \\
        & AP & \textbf{.504} & .068 & .390 & .467 & .093 & .398 \\ \midrule
        \multirow{2}{*}{ Pe } & F2 & .548 & .152 & .475 & \textbf{.486} & .213 & .487 \\
        & AP & .370 & .053 & .333 & \textbf{.397} & .120 & .375 \\ \midrule
        \multirow{2}{*}{ \textbf{Avg.} } & F2 & .362 & .187 & .335 & \textbf{.384} & .218 & .356 \\
        & AP & .275 & .066 & .247 & \textbf{.288} & .101 & .259 \\
        \bottomrule
        \end{tabular}
   
    \label{tab:exp2-results}
\end{table}



==> tables/exp3_table.tex <==
 \begin{table}[ht!]
    \centering
     \caption{Average F2 and AP scores for six different techniques applied to synthesized IBAD datasets for 8 languages}
    \begin{tabular}{cc cccccc}
    \toprule
    & & \multicolumn{3}{c}{ Intermingled } & \multicolumn{3}{c}{ Translated } \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    & & CLWE-G & LDA & VSM & WE-G & LDA & VSM \\          \midrule
    \multirow{2}{*}{ De } & F2 & \textbf{.343} & .167 & .297 & .342 & .207 & .325 \\
    & AP & .237 & .055 & .207 & \textbf{.239} & .075 & .226 \\  \midrule
    \multirow{2}{*}{ Fr } & F2 & \textbf{.350} & .188 & .303 & .340 & .198 & .328 \\
    & AP & .234 & .057 & .209 & \textbf{.240} & .068 & .234 \\ \midrule
    \multirow{2}{*}{ Hu } & F2 & .325 & .174 & .275 & \textbf{.332} & .208 & .318 \\
    & AP & .219 & .055 & .194 & \textbf{.231} & .072 & .221 \\ \midrule
    \multirow{2}{*}{ It } & F2 & \textbf{.341}& .176 & .303 & .342 & .201 & .322 \\
    & AP & .232 & .064 & .207 & \textbf{.245} & .070 & .230 \\ \midrule
    \multirow{2}{*}{ Ru } & F2 & .329 & .188 & .311 & \textbf{.337} & .177 & .321 \\
    & AP & .208 & .077 & .204 & \textbf{.241} & .057 & .217 \\ \midrule
    \multirow{2}{*}{ Sk } & F2 & .310 & .160 & .263 & \textbf{.327} & .193 & .292 \\
    & AP & .204 & .049 & .186 & \textbf{.223} & .068 & .206 \\ \midrule
    \multirow{2}{*}{ Sv } & F2 & .330 & .167 & .285 & \textbf{.340} & .186 & .322 \\
    & AP & \textbf{.238} & .064 & .203 & .237 & .068 & .224 \\ \midrule
    \multirow{2}{*}{ Tr } & F2 & .323 & .165 & .278 & \textbf{.349} & .190 & .325 \\
    & AP & .228 & .043 & .196 & \textbf{.247} & .064 & .221 \\ \midrule
    \multirow{2}{*}{ \textbf{Avg.}} & F2 & 0.332 & 0.173 & 0.289 & \textbf{0.339} & 0.195 & 0.319 \\
    & AP & .225 & .058 & .201 & \textbf{.238} & .068 & .222 \\
    \bottomrule
    \end{tabular}
   
    \label{tab:exp3-results}
\end{table}
